Aharonov-Bohm interference and phase-coherent surface-state transport in topological insulator rings

We present low-temperature magnetotransport measurements on selectively-grown Sb$_2$Te$_3$-based topological insulator ring structures. These topological insulator ring geometries display clear Aharonov-Bohm oscillations in the conductance originating from phase-coherent transport around the ring. The temperature dependence of the oscillation amplitude indicates that the Aharonov-Bohm oscillations originate from ballistic transport along the ring arms. The oscillations can therefore be attributed to topological surface states, which can maintain a quasi-ballistic transport regime in the presence of disorder. Further insight on the phase coherence is gained by comparing with similar Aharonov-Bohm-type oscillations in topological insulator nanoribbons exposed to an axial magnetic field. Here, quasi-ballistic phase-coherent transport is confirmed for closed-loop topological surface states in transverse direction enclosing the cross-section of the nanoribbon. In contrast, the appearance of universal conductance fluctuations indicates phase-coherent transport in the diffuse regime, which is attributed to bulk carrier transport. Thus, it appears that even in the presence of diffusive $p$-type charge carriers in Aharonov-Bohm ring structures, phase-coherent quasi-ballistic transport of topologically protected surface states is maintained over long distances.

==> abstract.tex <==
\begin{abstract}
We present low-temperature magnetotransport measurements on selectively-grown Sb$_2$Te$_3$-based topological insulator ring structures. These topological insulator  ring geometries display clear Aharonov-Bohm  oscillations in the conductance originating from phase-coherent transport around the ring. The temperature dependence of the oscillation amplitude indicates that the Aharonov-Bohm oscillations originate from ballistic transport along the ring arms. The oscillations can therefore be attributed to topological surface states, which can maintain a quasi-ballistic transport regime in the presence of disorder. Further insight on the phase coherence is gained by comparing with similar Aharonov-Bohm-type oscillations in topological insulator  nanoribbons exposed to an axial magnetic field. Here, quasi-ballistic phase-coherent transport is confirmed for closed-loop topological surface states in transverse direction enclosing the cross-section of the nanoribbon. In contrast, the appearance of universal conductance fluctuations indicates phase-coherent transport in the diffuse regime, which is attributed to bulk carrier transport. Thus, it appears that even in the presence of diffusive $p$-type charge carriers in Aharonov-Bohm ring structures, phase-coherent quasi-ballistic transport of topologically protected surface states is maintained over long distances.
\end{abstract}
